Generative Adversarial Networks for Extreme Learned Image Compression

We present a learned image compression system based on GANs, operating at extremely low bitrates. Our proposed framework combines an encoder, decoder/generator and a multi-scale discriminator, which we train jointly for a generative learned compression objective. The model synthesizes details it cannot afford to store, obtaining visually pleasing results at bitrates where previous methods fail and show strong artifacts. Furthermore, if a semantic label map of the original image is available, our method can fully synthesize unimportant regions in the decoded image such as streets and trees from the label map, proportionally reducing the storage cost. A user study confirms that for low bitrates, our approach is preferred to state-of-the-art methods, even when they use more than double the bits.

==> fig_full_4chan.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{ccc}
%\multicolumn{3}{c}{Synthesize \emph{sky, vegetation, sidewalk, ego vehicle, wall} in addition to:} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.33\linewidth]{figs/synth_classes/us1.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.082500\linewidth]{figs/synth_classes/us1_hm.jpg}}}
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{figs/synth_classes/us2.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.082500\linewidth]{figs/synth_classes/us2_hm.jpg}}}
\end{overpic} &
%
\includegraphics[width=0.33\linewidth]{figs/synth_classes/bpg.jpg} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
base ($0.062$ bpp) & +\emph{buildings} ($0.038$ bpp) & BPG ($0.043$ bpp)\vspace{0.6ex}
%
\end{tabular}



==> fig_full_4chan_base.tex <==
OUTDIR=synth_classes
\begin{tabular}{ccc}
%\multicolumn{3}{c}{Synthesize \emph{sky, vegetation, sidewalk, ego vehicle, wall} in addition to:} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,road,sidewalk,parking,vegetation,sky/test_50/images/frankfurt_000000_018797_0.06234bpp_synthesized_image.jpg O=us1}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,road,sidewalk,parking,building,vegetation,sky/test_50/images/frankfurt_000000_018797_0.03809bpp_synthesized_image.jpg O=us2}
HEATMAP25
\end{overpic} &
%
\includegraphics[width=0.33\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/cityscapes/frankfurt_000000_018797_leftImg8bit_bpg_50_0.0432.png O=bpg} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
base (BPP0 bpp) & +\emph{buildings} (BPP1 bpp) & BPG (BPP2 bpp)\vspace{0.6ex}
%
\end{tabular}



==> fig_full_ade.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{cccc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{4ex}{%
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade/ade1.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade/ade1_hm.jpg}}}
\end{overpic}} &
\raisebox{3ex}{%
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade/ade2.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade/ade2_hm.jpg}}}
\end{overpic}} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade/ade3.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade/ade3_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade/ade4.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade/ade4_hm.jpg}}}
\end{overpic}
\end{tabular}



==> fig_full_ade_2.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{cccc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_2/ade1.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_2/ade1_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_2/ade2.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_2/ade2_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_2/ade3.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_2/ade3_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_2/ade4.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_2/ade4_hm.jpg}}}
\end{overpic} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.24\linewidth]{figs/synth_ade_2/orig1.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_2/orig2.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_2/orig3.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_2/orig4.jpg} 
\end{tabular}



==> fig_full_ade_2_base.tex <==
OUTDIR=synth_ade_2
MAKE_SQUARE
\begin{tabular}{cccc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000040_0.02604bpp_synthesized_image.jpg O=ade1}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000068_0.09059bpp_synthesized_image.jpg O=ade2}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000104_0.11544bpp_synthesized_image.jpg O=ade3}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000112_0.02740bpp_synthesized_image.jpg O=ade4}
HEATMAP20
\end{overpic} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000040_0.02604bpp_real_image.jpg O=orig1} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000068_0.09059bpp_real_image.jpg O=orig2} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000104_0.11544bpp_real_image.jpg O=orig3} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000112_0.02740bpp_real_image.jpg O=orig4} 
\end{tabular}



==> fig_full_ade_3.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{cccc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_3/ade5.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_3/ade5_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_3/ade6.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_3/ade6_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_3/ade7.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_3/ade7_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_3/ade8.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_3/ade8_hm.jpg}}}
\end{overpic} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.24\linewidth]{figs/synth_ade_3/orig5.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_3/orig6.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_3/orig7.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_3/orig8.jpg}
\end{tabular}



==> fig_full_ade_3_base.tex <==
OUTDIR=synth_ade_3
MAKE_SQUARE
\begin{tabular}{cccc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000244_0.02239bpp_synthesized_image.jpg O=ade5}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000272_0.04594bpp_synthesized_image.jpg O=ade6}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000508_0.04205bpp_synthesized_image.jpg O=ade7}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00001416_0.10756bpp_synthesized_image.jpg O=ade8}
HEATMAP20
\end{overpic} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000244_0.02239bpp_real_image.jpg O=orig5} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000272_0.04594bpp_real_image.jpg O=orig6} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000508_0.04205bpp_real_image.jpg O=orig7} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00001416_0.10756bpp_real_image.jpg O=orig8}
\end{tabular}



==> fig_full_ade_base.tex <==
OUTDIR=synth_ade
\begin{tabular}{cccc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\raisebox{4ex}{%
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000144_0.02891bpp_synthesized_image.jpg O=ade1}
HEATMAP20
\end{overpic}} &
\raisebox{3ex}{%
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3/test_latest/images/ADE_val_00000568_0.02422bpp_synthesized_image.jpg O=ade2}
HEATMAP20
\end{overpic}} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000100_0.04868bpp_synthesized_image.jpg O=ade3}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00001900_0.04096bpp_synthesized_image.jpg O=ade4}
HEATMAP20
\end{overpic}
\end{tabular}



==> fig_full_ade_boxes.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{cccc}
%
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_boxes/box1.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_boxes/box1_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_boxes/box2.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_boxes/box2_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_boxes/box3.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_boxes/box3_hm.jpg}}}
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{figs/synth_ade_boxes/box4.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.048000\linewidth]{figs/synth_ade_boxes/box4_hm.jpg}}}
\end{overpic} \\
%
%
\includegraphics[width=0.24\linewidth]{figs/synth_ade_boxes/orig1.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_boxes/orig2.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_boxes/orig3.jpg} &
\includegraphics[width=0.24\linewidth]{figs/synth_ade_boxes/orig4.jpg}
%
%
\end{tabular}



==> fig_full_ade_boxes_base.tex <==
OUTDIR=synth_ade_boxes
MAKE_SQUARE
\begin{tabular}{cccc}
%
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000392_0.07320bpp_synthesized_image.jpg O=box1}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000532_0.07893bpp_synthesized_image.jpg O=box2}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000908_0.07116bpp_synthesized_image.jpg O=box3}
HEATMAP20
\end{overpic} &
\begin{overpic}[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000980_0.07817bpp_synthesized_image.jpg O=box4}
HEATMAP20
\end{overpic} \\
%
%
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000392_0.07320bpp_real_image.jpg O=orig1} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000532_0.07893bpp_real_image.jpg O=orig2} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000908_0.07116bpp_real_image.jpg O=orig3} &
\includegraphics[width=0.24\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/ade20k_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3/test_latest/images/ADE_val_00000980_0.07817bpp_real_image.jpg O=orig4}
%
%
\end{tabular}



==> fig_full_boxes.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{ccc}
%
\includegraphics[width=0.32\linewidth]{figs/synth_boxes/orig.jpg} &
%
\begin{overpic}[width=0.32\linewidth]{figs/synth_boxes/box1.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.064000\linewidth]{figs/synth_boxes/box1_hm.jpg}}}
\end{overpic} &
%
\begin{overpic}[width=0.32\linewidth]{figs/synth_boxes/box2.jpg}
\put(1,1){\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.2pt}\fbox{\includegraphics[width=0.064000\linewidth]{figs/synth_boxes/box2_hm.jpg}}}
\end{overpic} \vspace{-0.9ex} \\
Original & $0.103$bpp & $0.103$bpp
%
\end{tabular}



==> fig_full_boxes_2_base.tex <==
OUTDIR=synth_boxes_2
\begin{tabular}{ccc}
%
\includegraphics[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.1,0.1,0.4,0.4/test_50/images/frankfurt_000001_047178_0.08130bpp_real_image.jpg O=origa} &
%
\begin{overpic}[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.1,0.1,0.4,0.4/test_50/images/frankfurt_000001_047178_0.08130bpp_synthesized_image.jpg O=box1}
HEATMAP20
\end{overpic} &
%
\begin{overpic}[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.5,0.5,0.4,0.4/test_50/images/frankfurt_000001_047178_0.08130bpp_synthesized_image.jpg O=box2}
HEATMAP20
\end{overpic} \\
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\includegraphics[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.1,0.5,0.4,0.4/test_50/images/munster_000008_000019_0.08367bpp_real_image.jpg O=origb} &
%
\begin{overpic}[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.1,0.5,0.4,0.4/test_50/images/munster_000008_000019_0.08367bpp_synthesized_image.jpg O=box3}
HEATMAP20
\end{overpic} &
%
\begin{overpic}[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.5,0.1,0.4,0.4/test_50/images/munster_000008_000019_0.08367bpp_synthesized_image.jpg O=box4}
HEATMAP20
\end{overpic} \\
%
% Bpp is BPP0
%
\end{tabular}



==> fig_full_boxes_base.tex <==
OUTDIR=synth_boxes
\begin{tabular}{ccc}
%
\includegraphics[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.1,0.1,0.4,0.4/test_50/images/frankfurt_000001_067092_0.10304bpp_real_image.jpg O=orig} &
%
\begin{overpic}[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.1,0.1,0.4,0.4/test_50/images/frankfurt_000001_067092_0.10304bpp_synthesized_image.jpg O=box1}
HEATMAP20
\end{overpic} &
%
\begin{overpic}[width=0.32\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_box_dsquant_3_box0.1,0.5,0.4,0.4/test_50/images/frankfurt_000001_067092_0.10304bpp_synthesized_image.jpg O=box2}
HEATMAP20
\end{overpic} \vspace{-0.9ex} \\
Original & BPP0bpp & BPP0bpp
%
\end{tabular}



==> fig_full_classes_2_base.tex <==
OUTDIR=synth_classes_3
\begin{tabular}{ccc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,road,sidewalk,wall,fence,vegetation,sky/test_50/images/frankfurt_000000_011810_0.07660bpp_synthesized_image.jpg O=road2}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,sidewalk,wall,fence,vegetation,sky,car/test_50/images/frankfurt_000000_011810_0.10804bpp_synthesized_image.jpg O=car2}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_unlabeled,ego%20vehicle,rectification%20border,out%20of%20roi,static,d/images/frankfurt_000000_011810_0.04105bpp_synthesized_image.jpg O=everything2}
HEATMAP25
\end{overpic} \vspace{-2.6ex} \\
\emph{road} (BPP0 bpp) & \emph{car}  (BPP1 bpp) & everything (BPP2 bpp)    \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,sidewalk,wall,fence,vegetation,sky,person/test_50/images/frankfurt_000000_011810_0.12023bpp_synthesized_image.jpg O=people2}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,sidewalk,building,wall,fence,vegetation,sky/test_50/images/frankfurt_000000_011810_0.11042bpp_synthesized_image.jpg O=building2}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_rail%20track/test_50/images/frankfurt_000000_011810_0.18617bpp_synthesized_image.jpg O=nothing2}
HEATMAP25
\end{overpic} \vspace{-2.6ex} \\
\emph{people} (BPP3 bpp) & \emph{building}  (BPP4 bpp) & no synth (BPP5 bpp) 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\\
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,road,sidewalk,wall,fence,vegetation,sky/test_50/images/frankfurt_000000_001751_0.09211bpp_synthesized_image.jpg O=road}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,sidewalk,wall,fence,vegetation,sky,car/test_50/images/frankfurt_000000_001751_0.13428bpp_synthesized_image.jpg O=car}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_unlabeled,ego%20vehicle,rectification%20border,out%20of%20roi,static,d/images/frankfurt_000000_001751_0.03371bpp_synthesized_image.jpg O=everything}
HEATMAP25
\end{overpic} \vspace{-2.6ex} \\
\emph{road} (BPP6 bpp) & \emph{car}  (BPP7 bpp) & everything (BPP8 bpp)    \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,sidewalk,wall,fence,vegetation,sky,person/test_50/images/frankfurt_000000_001751_0.14707bpp_synthesized_image.jpg O=people}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_ego%20vehicle,rectification%20border,sidewalk,building,wall,fence,vegetation,sky/test_50/images/frankfurt_000000_001751_0.11910bpp_synthesized_image.jpg O=building}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_rail%20track/test_50/images/frankfurt_000000_001751_0.17883bpp_synthesized_image.jpg O=nothing}
HEATMAP25
\end{overpic} \vspace{-2.6ex} \\
\emph{people} (BPP9 bpp) & \emph{building}  (BPP10 bpp) & no synth (BPP11 bpp) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}



==> fig_full_classes_base.tex <==
OUTDIR=synth_classes
\begin{tabular}{ccc}
%\multicolumn{3}{c}{Synthesize \emph{sky, vegetation, sidewalk, ego vehicle, wall} in addition to:} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.325\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3_ego%20vehicle,road,sidewalk,parking,wall,vegetation,sky/test_50/images/frankfurt_000000_014480_0.14591bpp_synthesized_image.jpg O=road}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.325\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3_ego%20vehicle,sidewalk,wall,vegetation,sky,car,truck,bus,caravan,motorcycle,bicycle/test_50/images/frankfurt_000000_014480_0.22699bpp_synthesized_image.jpg O=cars}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.325\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3_unlabe/test_50/images/frankfurt_000000_014480_0.03543bpp_synthesized_image.jpg O=everything}
HEATMAP25
\end{overpic} \\[-3pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\emph{road} (BPP0 bpp, -55\%) & \emph{car} (BPP1 bpp, -15\%) & everything (BPP2 bpp, -89\%)   \\[3pt]
%
\begin{overpic}[width=0.325\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3_ego%20vehicle,sidewalk,wall,vegetation,sky,person,rider/test_50/images/frankfurt_000000_014480_0.21895bpp_synthesized_image.jpg O=person}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.325\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3_ego%20vehicle,sidewalk,building,wall,fence,vegetation,sky/test_50/images/frankfurt_000000_014480_0.19889bpp_synthesized_image.jpg O=building}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.325\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_8ch_heat_map_mask_bn8_hm_type_instance_dsquant_3_rail%20track/test_50/images/frankfurt_000000_014480_0.32567bpp_synthesized_image.jpg O=nothing}
HEATMAP25
\end{overpic}  \\[-3pt]
\emph{people} (BPP3 bpp, -33\%) & \emph{building} (BPP4 bpp, -39\%) & no synth.\ (BPP5 bpp, -0\%)
%
\end{tabular}



==> fig_full_zoom.tex <==
% THIS FILE IS AUTOGENERATED do not change
\centering
\begin{tikzpicture}[zoomboxarray]
    \node [image node] { \includegraphics[width=0.45\textwidth]{figs/synth_zoom/img32.jpg} };
    \zoombox{0.175,0.9}
    \zoombox[magnification=2]{0.7,0.6}
    \zoombox{0.15,0.3}
    \zoombox[magnification=10]{0.86,0.35}
\end{tikzpicture}


==> fig_kodak_forest.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{cc}
%
\includegraphics[width=0.49\linewidth]{figs/kodak_forest_custom/kodim13.png} &
\includegraphics[width=0.49\linewidth]{figs/partial_kodak_forest/us.jpg} \vspace{-2.6ex} \\
Kodak Image 13 & Ours ($0.031$bpp)\\
%
\includegraphics[width=0.49\linewidth]{figs/partial_kodak_forest/bpg.jpg} &
\includegraphics[width=0.49\linewidth]{figs/kodak_forest_custom/kodim13_out_jp2k_0_037.jpg} \vspace{-2.6ex} \\
BPG ($0.073$bpp) & JPEG2000 ($0.037$bpp)\\
%
\includegraphics[width=0.49\linewidth]{figs/kodak_forest_custom/kodim13_webp_0_192.jpg} &
\includegraphics[width=0.49\linewidth]{figs/kodak_forest_custom/kodim13_out_jp_0_284.jpg} \vspace{-2.6ex} \\
WebP ($0.192$bpp) & JPEG ($0.248$bpp) 
%
\end{tabular}


==> fig_kodak_forest_base.tex <==
OUTDIR=partial_kodak_forest
\begin{tabular}{cc}
%
\includegraphics[width=0.49\linewidth]{figs/kodak_forest_custom/kodim13.png} &
\includegraphics[width=0.49\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_results/openimages_GC_60ch_NL_MSE10_BN4_LEVELS5no_IN200918_kodakperchannel/test_iter_140000/images/kodim13_0.03149bpp_synthesized_image.jpg O=us} \vspace{-2.6ex} \\
Kodak Image 13 & Ours (BPP0bpp)\\
%
\includegraphics[width=0.49\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim13_bpg_50_0.0727.png O=bpg} &
\includegraphics[width=0.49\linewidth]{figs/kodak_forest_custom/kodim13_out_jp2k_0_037.jpg} \vspace{-2.6ex} \\
BPG (BPP1bpp) & JPEG2000 ($0.037$bpp)\\
%
\includegraphics[width=0.49\linewidth]{figs/kodak_forest_custom/kodim13_webp_0_192.jpg} &
\includegraphics[width=0.49\linewidth]{figs/kodak_forest_custom/kodim13_out_jp_0_284.jpg} \vspace{-2.6ex} \\
WebP ($0.192$bpp) & JPEG ($0.248$bpp) 
%
\end{tabular}


==> fig_kodak_tall_1.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim04} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_1/ours1.jpg} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_1/bpg1.jpg} \vspace{-2.6ex} \\
Kodak Image 4 & Ours ($0.036$bpp) & BPG ($0.037$bpp)  \\
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim09} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_1/ours2.jpg} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_1/bpg2.jpg} \vspace{-2.6ex} \\
Kodak Image 9 & Ours ($0.036$bpp) & BPG ($0.037$bpp)  \\
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim10} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_1/ours3.jpg} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_1/bpg3.jpg} \vspace{-2.6ex} \\
Kodak Image 10 & Ours ($0.036$bpp) & BPG ($0.038$bpp)  \\
%
\end{tabular}


==> fig_kodak_tall_1_base.tex <==
OUTDIR=partial_kodak_tall_1
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim04} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim04_0.03600bpp_synthesized_image.jpg O=ours1} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim04_bpg_47_0.0366.png O=bpg1} \vspace{-2.6ex} \\
Kodak Image 4 & Ours (BPP0bpp) & BPG (BPP1bpp)  \\
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim09} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim09_0.03600bpp_synthesized_image.jpg O=ours2} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim09_bpg_48_0.0370.png O=bpg2} \vspace{-2.6ex} \\
Kodak Image 9 & Ours (BPP0bpp) & BPG (BPP3bpp)  \\
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim10} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim10_0.03600bpp_synthesized_image.jpg O=ours3} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim10_bpg_48_0.0385.png O=bpg3} \vspace{-2.6ex} \\
Kodak Image 10 & Ours (BPP0bpp) & BPG (BPP5bpp)  \\
%
\end{tabular}


==> fig_kodak_tall_2.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim17} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_2/ours1.jpg} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_2/bpg1.jpg} \vspace{-2.6ex} \\
Kodak Image 17 & Ours ($0.036$bpp) & BPG ($0.039$bpp)  \\
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim18} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_2/ours2.jpg} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_2/bpg2.jpg} \vspace{-2.6ex} \\
Kodak Image 18 & Ours ($0.036$bpp) & BPG ($0.040$bpp)  \\
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim19} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_2/ours3.jpg} &
\includegraphics[width=0.22\linewidth]{figs/partial_kodak_tall_2/bpg3.jpg} \vspace{-2.6ex} \\
Kodak Image 19 & Ours ($0.036$bpp) & BPG ($0.036$bpp)  \\
%
\end{tabular}


==> fig_kodak_tall_2_base.tex <==
OUTDIR=partial_kodak_tall_2
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim17} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim17_0.03600bpp_synthesized_image.jpg O=ours1} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim17_bpg_49_0.0392.png O=bpg1} \vspace{-2.6ex} \\
Kodak Image 17 & Ours (BPP0bpp) & BPG (BPP1bpp)  \\
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim18} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim18_0.03600bpp_synthesized_image.jpg O=ours2} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim18_bpg_50_0.0397.png O=bpg2} \vspace{-2.6ex} \\
Kodak Image 18 & Ours (BPP0bpp) & BPG (BPP3bpp)  \\
%
%
\includegraphics[width=0.22\linewidth]{figs/kodak_orig/kodak_tall/kodim19} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim19_0.03600bpp_synthesized_image.jpg O=ours3} &
\includegraphics[width=0.22\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim19_bpg_50_0.0358.png O=bpg3} \vspace{-2.6ex} \\
Kodak Image 19 & Ours (BPP0bpp) & BPG (BPP5bpp)  \\
%
\end{tabular}


==> fig_kodak_wide_1.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim01} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/ours1.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/bpg1.jpg} \vspace{-2.6ex} \\
Kodak Image 1 & Ours ($0.036$bpp) & BPG ($0.043$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim02} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/ours2.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/bpg2.jpg} \vspace{-2.6ex} \\
Kodak Image 2 & Ours ($0.036$bpp) & BPG ($0.039$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim03} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/ours3.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/bpg3.jpg} \vspace{-2.6ex} \\
Kodak Image 3 & Ours ($0.036$bpp) & BPG ($0.035$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim05} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/ours5.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/bpg5.jpg} \vspace{-2.6ex} \\
Kodak Image 5 & Ours ($0.036$bpp) & BPG ($0.082$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim06} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/ours6.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_1/bpg6.jpg} \vspace{-2.6ex} \\
Kodak Image 6 & Ours ($0.036$bpp) & BPG ($0.033$bpp)  \\
%
\end{tabular}


==> fig_kodak_wide_2.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim07} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/ours0.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/bpg0.jpg} \vspace{-2.6ex} \\
Kodak Image 7 & Ours ($0.036$bpp) & BPG ($0.038$bpp)  \\
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim08} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/ours1.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/bpg1.jpg} \vspace{-2.6ex} \\
Kodak Image 8 & Ours ($0.036$bpp) & BPG ($0.040$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim11} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/ours2.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/bpg2.jpg} \vspace{-2.6ex} \\
Kodak Image 11 & Ours ($0.036$bpp) & BPG ($0.098$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim12} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/ours3.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/bpg3.jpg} \vspace{-2.6ex} \\
Kodak Image 12 & Ours ($0.036$bpp) & BPG ($0.038$bpp)  \\
%
%%%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim14} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/ours5.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/bpg5.jpg} \vspace{-2.6ex} \\
Kodak Image 14 & Ours ($0.036$bpp) & BPG ($0.038$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim15} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/ours6.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_2/bpg6.jpg} \vspace{-2.6ex} \\
Kodak Image 15 & Ours ($0.036$bpp) & BPG ($0.050$bpp)  \\
%
%
\end{tabular}


==> fig_kodak_wide_2_base.tex <==
OUTDIR=partial_kodak_wide_2
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim07} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim07_0.03600bpp_synthesized_image.jpg O=ours0} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim07_bpg_50_0.0401.png O=bpg0} \vspace{-2.6ex} \\
Kodak Image 7 & Ours (BPP0bpp) & BPG (BPP11bpp)  \\
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim08} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim08_0.03600bpp_synthesized_image.jpg O=ours1} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim08_bpg_50_0.0978.png O=bpg1} \vspace{-2.6ex} \\
Kodak Image 8 & Ours (BPP0bpp) & BPG (BPP1bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim11} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim11_0.03600bpp_synthesized_image.jpg O=ours2} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim11_bpg_49_0.0378.png O=bpg2} \vspace{-2.6ex} \\
Kodak Image 11 & Ours (BPP0bpp) & BPG (BPP3bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim12} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim12_0.03600bpp_synthesized_image.jpg O=ours3} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim12_bpg_45_0.0380.png O=bpg3} \vspace{-2.6ex} \\
Kodak Image 12 & Ours (BPP0bpp) & BPG (BPP5bpp)  \\
%
%%%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim14} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim14_0.03600bpp_synthesized_image.jpg O=ours5} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim14_bpg_50_0.0499.png O=bpg5} \vspace{-2.6ex} \\
Kodak Image 14 & Ours (BPP0bpp) & BPG (BPP7bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim15} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim15_0.03600bpp_synthesized_image.jpg O=ours6} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim15_bpg_47_0.0383.png O=bpg6} \vspace{-2.6ex} \\
Kodak Image 15 & Ours (BPP0bpp) & BPG (BPP9bpp)  \\
%
%
\end{tabular}


==> fig_kodak_wide_3.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim16} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/ours0.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/bpg0.jpg} \vspace{-2.6ex} \\
Kodak Image 16 & Ours ($0.036$bpp) & BPG ($0.050$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim20} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/ours1.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/bpg1.jpg} \vspace{-2.6ex} \\
Kodak Image 20 & Ours ($0.036$bpp) & BPG ($0.039$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim21} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/ours2.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/bpg2.jpg} \vspace{-2.6ex} \\
Kodak Image 21 & Ours ($0.036$bpp) & BPG ($0.036$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim22} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/ours3.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/bpg3.jpg} \vspace{-2.6ex} \\
Kodak Image 22 & Ours ($0.036$bpp) & BPG ($0.043$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim23} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/ours5.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/bpg5.jpg} \vspace{-2.6ex} \\
Kodak Image 23 & Ours ($0.036$bpp) & BPG ($0.038$bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim24} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/ours6.jpg} &
\includegraphics[width=0.30\linewidth]{figs/partial_kodak_wide_3/bpg6.jpg} \vspace{-2.6ex} \\
Kodak Image 24 & Ours ($0.036$bpp) & BPG ($0.037$bpp)  \\
%
%
\end{tabular}


==> fig_kodak_wide_3_base.tex <==
OUTDIR=partial_kodak_wide_3
\begin{tabular}{ccc}
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim16} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim16_0.03600bpp_synthesized_image.jpg O=ours0} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim16_bpg_46_0.0388.png O=bpg0} \vspace{-2.6ex} \\
Kodak Image 16 & Ours (BPP0bpp) & BPG (BPP11bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim20} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim20_0.03600bpp_synthesized_image.jpg O=ours1} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim20_bpg_48_0.0359.png O=bpg1} \vspace{-2.6ex} \\
Kodak Image 20 & Ours (BPP0bpp) & BPG (BPP1bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim21} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim21_0.03600bpp_synthesized_image.jpg O=ours2} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim21_bpg_50_0.0426.png O=bpg2} \vspace{-2.6ex} \\
Kodak Image 21 & Ours (BPP0bpp) & BPG (BPP3bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim22} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim22_0.03600bpp_synthesized_image.jpg O=ours3} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim22_bpg_48_0.0379.png O=bpg3} \vspace{-2.6ex} \\
Kodak Image 22 & Ours (BPP0bpp) & BPG (BPP5bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim23} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim23_0.03600bpp_synthesized_image.jpg O=ours5} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim23_bpg_48_0.0367.png O=bpg5} \vspace{-2.6ex} \\
Kodak Image 23 & Ours (BPP0bpp) & BPG (BPP7bpp)  \\
%
%
\includegraphics[width=0.30\linewidth]{figs/kodak_orig/kodak_wide/kodim24} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_kodak/ade20k_512p_globalcompression_mse_4ch_nolabels_Dkodak_blur/test_50/images/kodim24_0.03600bpp_synthesized_image.jpg O=ours6} &
\includegraphics[width=0.30\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/kodak_bpg/kodim24_bpg_50_0.0500.png O=bpg6} \vspace{-2.6ex} \\
Kodak Image 24 & Ours (BPP0bpp) & BPG (BPP9bpp)  \\
%
%
\end{tabular}


==> fig_part_4ch_ade.tex <==
% THIS FILE IS AUTOGENERATED do not change
\begin{tabular}{cccc}
%
\includegraphics[width=0.24\columnwidth]{figs/partial_4ch_ade/img1_us.jpg} &
\includegraphics[width=0.24\columnwidth]{figs/partial_4ch_ade/img1_bpg.jpg} &
\includegraphics[width=0.24\columnwidth]{figs/partial_4ch_ade/img2_us.jpg} &
\includegraphics[width=0.24\columnwidth]{figs/partial_4ch_ade/img2_bpg.jpg} \\
Ours ($0.036$bpp) & BPG ($0.092$bpp) & Ours ($0.072$bpp) & BPG ($0.082$bpp)
%
%
\end{tabular}


==> fig_part_4ch_ade_base.tex <==
OUTDIR=partial_4ch_ade
\begin{tabular}{cccc}
%
\includegraphics[width=0.25\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_results/ade20k_512p_globalcompression_mse_4ch_nolabels_D/test_latest/images/ADE_val_00000020_0.03600bpp_synthesized_image.jpg O=img1_us} &
\includegraphics[width=0.25\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/sceneparse150_new_all/ADE_val_00000020_real_image_bpg_50_0.0924.png O=img1_bpg} &
\includegraphics[width=0.25\linewidth]{http://people.ee.ethz.ch/~aeirikur/pix2bits_results/ade20k_512p_globalcompression_mse_8ch_fix/test_10/images/ADE_val_00001288_0.07200bpp_synthesized_image.jpg O=img2_us} &
\includegraphics[width=0.25\linewidth]{http://people.ee.ethz.ch/~mentzerf/pix2bits_results/bpg/sceneparse150_new_all/ADE_val_00001288_real_image_bpg_49_0.0818.png O=img2_bpg} \\
Ours (BPP0bpp) & BPG (BPP1bpp) & Ours (BPP2bpp) & BPG (BPP3bpp)
%
%
\end{tabular}


==> fig_predicted_base.tex <==
OUTDIR=synth_classes_3
\begin{tabular}{ccc}
\includegraphics[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_reb/test_50/images/frankfurt_000001_004736_0.01921bpp_real_image.jpg O=gt1} &
    \includegraphics[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_reb/test_50/images/frankfurt_000001_028232_0.02125bpp_real_image.jpg} &
    \includegraphics[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_reb/test_50/images/frankfurt_000001_046272_0.01343bpp_real_image.jpg} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_reb/test_50/images/frankfurt_000001_004736_0.01921bpp_synthesized_image.jpg O=ex1}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_reb/test_50/images/frankfurt_000001_028232_0.02125bpp_synthesized_image.jpg O=ex2}
HEATMAP25
\end{overpic} &
%
\begin{overpic}[width=0.33\linewidth]{http://people.ee.ethz.ch/~michaelt/pix2bits_results/label2city_512p_globalcompressionlabel_mse10_4ch_heat_map_mask_bn4_hm_type_instance_dsquant_3_reb/test_50/images/frankfurt_000001_046272_0.01343bpp_synthesized_image.jpg O=ex3}
HEATMAP25
\end{overpic} \vspace{-2.6ex} \\
(BPP0 bpp) &  (BPP1 bpp) & (BPP2 bpp)    \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\end{tabular}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

